Quantitative Curve Selection Lemma

We prove a quantitative version of the curve selection lemma. Denoting by $s,d,k$ a bound on the number, the degree and the number of variables of the polynomials describing a semi-algebraic set $S$ and a point $x$ in $\bar S$, we find a semi-algebraic path starting at $x$ and entering in $S$ with a description of degree $(O(d)^{3k+3},O(d)^{k})$ (using a precise definition of the description of a semi-algebraic path and its degree given in the paper). As a consequence, we prove that there exists a semi-algebraic path starting at $x$ and entering in $S$, such that the degree of the Zariski closure of the image of this path is bounded by $O(d)^{4k+3}$, improving a result of Jelonek and Kurdyka. We also give an algorithm for describing the real isolated points of $S$ whose complexity is bounded by $s^{2 k+1}d^{O(k)}$ improving a result of Le, Safey el Din, and de Wolff.

==> BR-abbr.tex <==
%%BPR-abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand {\hide}[1]{}


%chapter 1
\newcommand {\Complex}[1]   {\mathrm{{\mathbb C}^{#1}}}
\newcommand {\C}     {\mathrm{C}}
\newcommand {\Real}[1]   {\mathrm{{\mathbb R}^{#1}}}
\newcommand {\ZZ} {\mathrm{Zer}}
\newcommand {\Free} {\mathrm{Free}}
\newcommand {\RR} {\mathrm{Reali}}
\newcommand {\Z}  {{\mathbb Z}}
\newcommand{\Qu} {\mathrm{Q}}
\newcommand {\D}     {\mathrm{D}}
\newcommand {\K}     {\mathrm{K}}
\newcommand {\Q}         {{\mathbb Q}}
\newcommand {\lc}       {\mathrm{lcof}}
\newcommand {\cf}     {\mathrm{cof}}
\newcommand {\complex}   {\Complex{}}
\newcommand {\rem}     {\mathrm{Rem}}
\newcommand {\quo}     {\mathrm{Quo}}
\newcommand {\lcm}      {\mathrm{lcm}}
\renewcommand {\E} {\mathrm{ExtsRem}}
\renewcommand {\SS} {\mathrm{sRem}}
\newcommand {\SU} {\mathrm{sRemU}}
\newcommand {\SV} {\mathrm{sRemV}}
\newcommand {\prem}     {\mathrm{Prem}}
\newcommand{\Tru}  {\mathrm{Tru}}
\newcommand {\sprem}     {\mathrm{sPrem}}
\newcommand {\paremseq} {\mathrm{TRems}}
\newcommand{\Po}  {\mathrm{Pol}}
\newcommand {\pagcd}    {\mathrm{Pgcd}}
\newcommand {\LTRem} {\mathrm{LTR}}
\newcommand {\TRem} {\mathrm{TRem}}
 \newcommand {\N}         {{\mathbb N}}

%chapter 2
\newcommand {\A}     {\mathrm{A}}
\newcommand{\F}{\mathrm{F}}
\newcommand {\sign}        {\mathrm{sign}}
\newcommand {\re}         {\Real{}}
\newcommand {\eps} {{\varepsilon}}
\newcommand {\R} {\mathrm{R}}
\newcommand {\alg} {\mathrm{alg}}
\newcommand {\lex} {\mathrm{lex}}
\newcommand {\grlex} {\mathrm{grlex}}
\newcommand {\Der} {\mathrm{Der}}
\newcommand {\V} {\mathrm{Var}}
\newcommand  {\pos} {\mathrm{pos}}
\newcommand {\num} {\mathrm{num}}
\newcommand {\numm} {\mathrm{nu}}
\newcommand {\Ind} {\mathrm{Ind}}
\newcommand {\TaQ} {\mathrm{TaQ}}
\newcommand {\Mat} {\mathrm{Mat}}
\newcommand {\Graph} {\mathrm{Graph}}
\newcommand {\Ext} {\mathrm{Ext}}
\newcommand {\la}   {{\langle}}
\newcommand {\ra}   {{\rangle}}
\newcommand {\In} {\mathrm{ini}}

%chapter 3
\newcommand {\Id} {\mathrm{Id}}
\newcommand {\Deri} {\mathrm{d}}

%chapter 4
\newcommand{\Disc}  {\mathrm{Disc}}
\newcommand{\sDisc}  {\mathrm{sDisc}}
\newcommand {\Newton}       {\mathrm{Newt}}
\newcommand {\Syl} {\mathrm{Syl}}
\newcommand {\Res}      {\mathrm{Res}}
\newcommand {\SH} {\mathrm{SylvHa}}
\newcommand {\sr} {\mathrm{sRes}}
\newcommand{\udots}{{\mathinner{\mskip1mu\raise1pt\vbox{\kern7pt\hbox{.}}\mskip2mu\raise4pt\hbox{.}\mskip2mu\raise7pt\hbox{.}\mskip1mu}}}
\newcommand{\longrightarrowlim}{\mathop{\longrightarrow}\limits}
\newcommand{\PMC}  {\mathrm{PmV}}
\newcommand{\Rank}  {\mathrm{Rank}}
\newcommand{\Sign}  {\mathrm{Sign}}
\newcommand {\Ker}      {\mathrm{Ker}}
\newcommand{\Tr}  {\mathrm{Tr}}
\newcommand{\charpoly}  {\mathrm{charpoly}}
\newcommand{\Sym}  {\mathrm{Sym}}
\newcommand{\Her}  {\mathrm{Her}}
\newcommand{\Ideal}  {\mathrm{Ideal}}
\newcommand {\revlex} {\mathrm{revlex}}
\newcommand {\lmon}      {\mathrm{lmon}}
\newcommand {\lt}      {\mathrm{lt}}
\newcommand {\Red} {\mathrm {Red}}
\newcommand {\LL}       {\mathrm{L}}
\newcommand {\Proj}       {\mathrm{Proj}}
\newcommand {\her}       {\mathrm{her}}
\newcommand {\Rad}       {\mathrm{Rad}}
\newcommand {\rad}       {\mathrm{rad}}
\newcommand {\PP}     {{\mathbb P}}

%chapter 5
\newcommand{\Elim}  {\mathrm{Elim}}
\newcommand{\ba}  {\mathrm{ba}}

%chapter 6
\newcommand{\Ch}  {\mathrm{Ch}}
\newcommand{\HH}{\mathrm{H}}
\newcommand{\be}  {\mathrm{b}}
\newcommand{\chiep}  {\mathrm{EPC}}
\newcommand{\starstar}  {\mathrm{star}}
\newcommand{\diam}  {\mathrm{diam}}
\newcommand{\mesh}  {\mathrm{mesh}}
\newcommand {\dist} {\mathrm{dist}}
\newcommand{\BM}  {\mathrm{BM}}
\newcommand{\EQ}  {\mathrm{EPQ}}

%chapter 7
\newcommand{\Grad}  {\mathrm{Grad}}
\newcommand{\Hes}  {\mathrm{Hes}}
\newcommand{\SIGN}  {\mathrm{SIGN}}
\newcommand{\Homotop}  {\mathrm{H}}
\newcommand{\level}  {\mathrm{level}}

%chapter 8
\newcommand {\bit} {\mathrm {bit}}
\newcommand{\Hor}  {\mathrm{Hor}}
\newcommand {\pdet} {\mathrm{pdet}}
\newcommand {\SR} {\mathrm{sResP}}
\newcommand{\SHPol}  {\mathrm{SHPol}}
\newcommand {\sResU} {\mathrm{sResU}}
\newcommand {\sResV} {\mathrm{sResV}}


%chapter 9
\newcommand {\W}      {\mathrm{MVar}}
\newcommand{\Bez}  {\mathrm{Bez}}
\newcommand{\HanB}  {\mathrm{HanB}}
\newcommand{\Han} {\mathrm{Han}}
\newcommand{\han} {\mathrm{han}}
\newcommand{\To}  {\mathrm{To}}

%chapter 10
\newcommand {\Le}       {\mathrm{L}}
\newcommand {\M}        {\mathrm{M}}
\newcommand{\cont}  {\mathrm{cont}}
\newcommand{\sep}  {\mathrm{sep}}
\newcommand{\Bern}  {\mathrm{Bern}}
\newcommand {\Rec}      {\mathrm{Rec}}
\newcommand {\Co}      {\mathrm{C}}
\newcommand {\T}      {\mathrm{T}}
\newcommand{\Pos}  {\mathrm{Pos}}
\newcommand{\NCom}  {\mathrm{NCom}}
\newcommand{\NN}  {\mathrm{NN}}
\newcommand{\Ada}  {\mathrm{Ada}}
\newcommand {\Comp} {\mathrm {Comp}}
\newcommand{\Used}  {\mathrm{Used}}
\newcommand{\Thom}  {\mathrm{Thom}}

%chapter 11
\newcommand{\size}  {\mathrm{size}}
\newcommand{\CF}  {\mathrm{CF}}
\newcommand{\CSign}  {\mathrm{CSign}}
\newcommand{\True}  {\mathrm{True}}
\newcommand{\False}  {\mathrm{False}}
\newcommand{\sDiscP}  {\mathrm{sDiscP}}
\newcommand{\RElim}  {\mathrm{RElim}}

%chapter 12
\newcommand{\Sy}  {\mathrm{S}}
\newcommand {\MUS}      {\mathrm{Und}}
\newcommand {\B} {\mathrm {Bor}}
\newcommand {\NF}       {\mathrm{NorF}}
\newcommand {\Def} {\mathrm {Def}}
\newcommand {\Cr} {\mathrm {Cr}}
\newcommand{\tdeg}  {\mathrm{tdeg}}
\newcommand{\Bor}  {\mathrm{Bor}}
\newcommand{\Mon}  {\mathrm{Mon}}
\newcommand{\Cor}  {\mathrm{Cor}}
\newcommand{\Tab}  {\mathrm{Tab}}
\newcommand{\Prop}  {\mathrm{Prop}}

%chapter 13
\newcommand{\App}  {\mathrm{App}}

%chapter 14
\newcommand{\BElim}  {\mathrm{BElim}}
\newcommand{\UR}  {\mathrm{UR}}
\newcommand{\Rem}  {\mathrm{Remo}}
\newcommand{\BB}  {\mathrm{BB}}
\newcommand{\SSign}  {\mathrm{SSign}}

%chapter 15
\newcommand{\RM}  {\mathrm{RM}}
\newcommand{\pr}  {\mathrm{Pr}}
\newcommand{\CS}  {\mathrm{CS}}


%chapter 16
\newcommand{\URM}  {\mathrm{URM}}
\newcommand{\Ima}  {\mathrm{Im}}

\hide{
\def\strictsubset{\mathrel{\mathop{\kern 0pt \SRbset}\limits_{\not=}}}
\newcommand {\pquo}     {\mathrm{Pquo}}
\newcommand {\parem}   {\mathrm{Parem}}
\newcommand {\posquo}   {\mathrm{Posquo}}
\newcommand {\posgcd}    {\mathrm{Posgcd}}
\newcommand {\SI}         {\mathrm{SIGN}_R}
\newcommand{\decide} {\mathrm{Decide}}
\renewcommand {\I} {\mathrm{I}}
\def\gau {\mathrm{Gau}}
\newcommand {\ldp}      {\mathrm{ldp}}
\newcommand {\GRem}      {\mathrm{GRem}}
\newcommand {\SB} {\mathrm{SB}}
\newcommand {\Ho}      {\mathrm{H}}
\newcommand{\epc}  {\mathrm{EPC}}
\def\addots{\mathinner{\mkern1mu
\raise1pt\vbox{\kern7pt\hbox{.}}
\mkern2mu\raise4pt\hbox{.}\mkern2mu
\raise7pt\hbox{.}\mkern1mu}}
\newcommand{\der}  {\mathrm{der}}
\newcommand{\Hom}  {\mathrm{Hom}}
\newcommand{\Feas}  {\mathrm{Feas}}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%BR-abbreviations

%% added 2017
%\newcommand{\MF}[1]{\textcolor{cyan}{\textsc{MF:} {\sf #1}}}
%\renewcommand{\sb}[1]{\textcolor{blue}{\textsc{sb:} {\sf #1}}}






